Monostability and bistability of biological switches

Cell-fate transition can be modeled by ordinary differential equations (ODEs) which describe the behavior of several molecules in interaction, and for which each stable equilibrium corresponds to a possible phenotype (or 'biological trait'). In this paper, we focus on simple ODE systems modeling two molecules which each negatively (or positively) regulate the other. It is well-known that such models may lead to monostability or multistability, depending on the selected parameters. However, extensive numerical simulations have led systems biologists to conjecture that in the vast majority of cases, there cannot be more than two stable points. Our main result is a proof of this conjecture. More specifically, we provide a criterion ensuring at most bistability, which is indeed satisfied by most commonly used functions. This includes Hill functions, but also a wide family of convex and sigmoid functions. We also determine which parameters lead to monostability, and which lead to bistability, by developing a more general framework encompassing all our results.

==> general_framework.tex <==
The first purpose of this section is to prove the first theorem of the previous section (Theorem~\ref{theo three-one}), which provides the parameter spaces for which system \eqref{initial system}  is monostable or bistable.  We will see that this result is part of a general framework, thank to which we can retrieve the result of the second section, which states that, under some hypothesis, system \eqref{initial system} cannot have more than two stable equilibria. 

We introduce a family of sets: for $n\in \mathbb{N}^*$, let
$$E_n:=\biggl\{(x,y)\in (\mathbb{R}_+^{n})^2 :\, \forall i\neq j,  \frac{x_i}{f(y_i)}=\frac{x_j}{f(y_j)}, \frac{y_i}{g(x_i)}=\frac{y_j}{g(x_j)}, \, x_i\neq x_j\biggr\}. $$
Notice that, since $f$ and $g$ are one-to-one, $E_n$ can also be written  
%%%
$$E_n=\biggl\{(x,y)\in (\mathbb{R}_+^{n})^2 :\, \forall i\neq j,  \frac{x_i}{f(y_i)}=\frac{x_j}{f(y_j)}, \frac{y_i}{g(x_i)}=\frac{y_j}{g(x_j)},\, y_i\neq y_j\biggr\}. $$
%%%
By convention, we take $E_1=\mathbb{R}_+^2$.
%%%
We also introduce two subsets of the above sets $E_n$:
%%%
\[E_n^>:=\biggl\{(x,y)\in E_n : \underset{i\in \{1,\ldots,n\}}\min\biggl(\frac{x_ig'(x_i)}{g(x_i)}\frac{y_if'(y_i)}{f(y_i)} \biggr)>1 \biggr\}\]
%%%
\[E_n^\geq:=\biggl\{(x,y)\in E_n : \underset{i\in \{1,\ldots,n\}}\min\biggl(\frac{x_ig'(x_i)}{g(x_i)}\frac{y_if'(y_i)}{f(y_i)} \biggr)\geq1 \biggr\}\]
%%%
We note that, in the particular case $n=1$, $E_1^\geq $ is the closure of $E_1^>$.

We also introduce 
\begin{align*}
G_n : E_n &\longrightarrow \mathbb{R}_+^2\\
 (x,y)&\longmapsto \biggl(\frac{x_i}{f(y_i)}, \frac{y_i}{g(x_i)}\biggr), 
\end{align*}
for some $i\in \{1,\ldots, n\}$. Remark that by the definition of $E_n$, the function $G_n$ is well-defined since the choice of $i$ is arbitrary. 


The following property explains how the sets $E_n^>$ and $E_n^\geq$ and the function $G_n$ may be used to study the number of equilibria of \eqref{initial system}. \\
\begin{prop}
Let $n\in \mathbb{N}^*$. 
\begin{itemize}
\item If $(\alpha, \beta)\in G_n(E_n^>)$, then system $\eqref{initial system}$ has at least $2n+1$ equilibria. 
\item If system $\eqref{initial system}$ has $2n$ equilibria or more, then $(\alpha, \beta)\in G_n({E_n^\geq})$ .
\end{itemize}
\label{E_n}
\end{prop}
There is a direct and useful consequence of this proposition:
\begin{cor}
If $E_n^>=\emptyset$, then for any choice of $\alpha$, $\beta$, system \eqref{initial system} has at most $2n-1$ equilibria.  
\label{cor empty}
\end{cor}

%\begin{prop}
%Let $n \in \mathbb{N}^*$. If 
%\[\underset{(x,y)\in E} {\sup}\biggl\{\underset{i\in \{1,...n\}}\min\biggl(\frac{x_if_2'(x_i)}%{f_2(x_i)}\frac{y_if_1'(y_i)}{f_1(y_i)} \biggr)\biggr\}>1,\]

%then there exist $g_1, g_2>0$ such that system \eqref{f param} has at least $2n+1$ equilibria. 

%Moreover, if system \eqref{f param} has $2n$ equilibria or more, then there exist $(x, y) \in E_n$ such that for a all $i \in \{1,...n\}$, 

%\[\frac{x_if_2'(x_i)}{f_2(x_i)}\frac{y_if_1'(y_i)}{f(y_i)}\geq 1\]

%\label{E_n}
%\end{prop}


\begin{proof}[Proof of Proposition \ref{E_n}]
Let us assume that $E_n^>\neq \emptyset$, and let $(\alpha, \beta) \in G_n(E_n^>)$. Then, there exists $(x, y) \in E_n$ such that, for all $i\in \{1,\ldots, n\}, $
\[\frac{ x_ig'(x_i)}{g( x_i)}\frac{ y_if'(y_i)}{f(y_i)}>1,\quad
\text{ and } \quad
\alpha=\frac{x_i}{f(y_i)}, \quad \beta=\frac{y_i}{g(x_i)}.
\]%%%
In other words, all the points $(x_i, y_i)$ are  equilibria of the system, and satisfy
$\alpha \beta f'(y_i)g'(x_i)>1.$
%%%
According to Corollary \ref{cor fixed points f positive},  this proves that $x\mapsto \alpha f(\beta g(x))$ has at least $2n+1$ fixed points, and thus that  system \eqref{initial system} has at least $2n+1$ equilibria. 

Now, let us assume that system \eqref{initial system} has at least $2n$ equilibria. According to Proposition \ref{prop fixed_point_derivative},   there exist at least $n$ of these equilibria (denoted $(\bar x_1, \bar y_1), \ldots, (\bar x_n, \bar y_n))$ which satisfy 
$\alpha \beta f'(\bar y_i)g'(\bar x_i)\geq 1.$
%%%
Since each $(\bar x_i, \bar y_i)$ is an equilibrium of \eqref{initial system}, then for all $i\in\{1,\cdots,n\}$,
\begin{align*}
\alpha =\frac{\bar x_i}{f(\bar y_i)}, \quad \beta =\frac{\bar y_i}{g(\bar x_i)}, 
\end{align*}
%%%
which proves that $(\alpha, \beta)\in G_n\bigl({E_n^\geq}\bigr).$
\end{proof}

Applying this proposition with $n=1$, we exactly get the result of the third section. 
If $n=2$, we get 
\[E_2=\biggl\{(x_1, x_2, y_1, y_2)\in \mathbb{R}_+^4 : \frac{x_1}{f(y_1)}= \frac{x_2}{f(y_2)}, \frac{y_1}{g(x_1)}=\frac{y_2}{g(x_2)}, \, x_1 \neq x_2\biggr\}, \]
%%%
and, since for any $(x_1, x_2, y_1, y_2)\in E_2$, 
\[\frac{x_i}{f(y_i)}= \frac{x_1-x_2}{f(y_1)-f(y_2)} \quad \text{and} \quad \frac{y_i}{g(x_i)}=\frac{y_1-y_2}{g(x_1)-g(x_2)}\]
%%%
we can rewrite 
\begin{align*}
E_2^\geq&=\biggl\{(x_1, x_2, y_1, y_2)\in E_2: \frac{\lvert x_1-x_2\rvert }{\lvert g(x_1)-g(x_2)\rvert } \frac{\lvert y_1-y_2\rvert }{\lvert f(y_1)-f(y_2)\rvert }\min\bigl(g'(x_1)f'(y_1), g'(x_2)f'(y_2) \bigr)\geq1 \biggr\}\\
&\subset \biggl\{(x_1, x_2, y_1, y_2)\in \mathbb{R}_+^4  \min\bigl(g'(x_1)f'(y_1), g'(x_2)f'(y_2) \bigr)\geq \frac{\lvert g(x_1)-g(x_2)\rvert}{\lvert x_1-x_2\rvert }\frac{\lvert f(y_1)-f(y_2)\rvert }{\lvert y_1-y_2\rvert } \biggr\}.
\end{align*}
%%%
Thus, if $f$ and $g$ are $\gamma^{1/2}$-convex, and one of these functions is strictly $\gamma^{1/2}$-convex, as seen in the second section (Proposition \ref{non-local}), we get,  for any $(x_1, x_2, y_1, y_4)\in \mathbb{R}_+^4$, 
\[f'(y_1)f'(y_2)\leq \biggl(\frac{f(y_2)-f(y_1)}{y_2-y_1}\biggr)^2 \quad \text{and} \quad g'(x_1)g'(x_2)\leq \biggl(\frac{g(x_2)-g(x_1)}{x_2-x_1}\biggr)^2,\]
%%%
(and one of this inequality is in fact strict)
and thus
\[g'(x_1)f'(y_1)f'(y_2)g'(x_2)< \biggl(\frac{\lvert g(x_1)-g(x_2)\rvert}{\lvert x_1-x_2\rvert}\frac{\lvert f(y_1)-f(y_2)\rvert }{\lvert y_1-y_2\rvert }\biggr)^2,\]
%%%
which proves that 
\[g'(x_1)f'(y_1)<\frac{\lvert g(x_1)-g(x_2)\rvert}{\lvert x_1-x_2\rvert}\frac{\lvert f(y_1)-f(y_2)\rvert }{\lvert y_1-y_2\rvert } \quad \text{or} \quad g'(x_2)f'(y_2)<\frac{\lvert g(x_1)-g(x_2)\rvert}{\lvert x_1-x_2\rvert}\frac{\lvert f(y_1)-f(y_2)\rvert }{\lvert y_1-y_2\rvert}, \]
%%%
and therefore that $E_2^\geq=\emptyset$ under this hypothesis. 




